Business Suitability Principles for Workflow Modelling

By incorporating aspects of coordination and collaboration, workflow implementations of information systems require a sound conceptualisation of \EM{business processing} semantics. Traditionally, the success of conceptual modelling techniques has depended largely on the adequacy of conceptualisation, expressive power, comprehensibility and formal foundation. An equally important requirement, particularly with the increased conceptualisation of business aspects, is \EM{business suitability}. In this paper, the focus is on the business suitability of workflow modelling for a commonly encountered class of (operational) business processing, e.g. those of insurance claims, bank loans and land conveyancing. A general assessment is first conducted on some \EM{integrated} techniques characterising well-known paradigms - structured process modelling, object-oriented modelling, behavioural process modelling and business-oriented modelling. Through this, an insight into business suitability within the broader perspective of technique adequacy, is gained. A specific business suitability diagnosis then follows using a particular characterisation of business processing, i.e.\ one where the intuitive semantics and inter-relationship of business services and business processes are nuanced. As a result, five business suitability principles are elicited. These are proposed for a more detailed understanding and (synthetic) development of workflow modelling techniques. Accordingly, further insight into workflow specification languages and workflow globalisation in open distributed architectures may also be gained.

==> btp01old.tex <==
\section{Introduction}
\label{intro}

The workflow concept, proliferated through the recently emergent
computer supported cooperative work (CSCW) systems and workflow
systems (see surveys in 
\cite{Report:94:Fitzpatrick:CSCW,%
Book:93:Wastell:CSCW,Article:91:Rodden:CSCW}
and
\cite{Article:95:Georgakopoulos:WFOverview} respectively), 
advances information systems (IS) implementation models by incorporating 
aspects of collaboration and coordination in business processes. Under 
traditional implementation models, applications are partitioned into 
discrete units of functionality, with (typically) operational procedures 
used to describe how human and computerised actions of business processes 
combine to deliver business services. Through an endowment of business 
process execution semantics, workflows permit a greater organisational 
fit of ISs. Moreover workflows are specified at a level above traditional 
applications, enabling program binding and access to a loosely-coupled set 
of databases and files. Therefore, newer applications may be developed out 
of existing applications to reflect reengineered business processes. 

Crucial to the specification of any IS implementation is the \EM{conceptual}
level. This, of course, orients the analysis of a given domain towards its
essence (deep-structure) rather than to aspects of implementation
(physical-structure) or representation (surface-structure). For workflows, the
standardisation of concepts is progressing through the Workflow Management
Coalition{\footnote{Refer to http://www.aiai.ed.ac.uk/WfMC/index.html for
more details.}}.
While the set of terms and references defined so far characterise
sufficiently the notion of workflow, e.g.\ event, process (including
pre-conditions, post-conditions and state transitions) and organisational
(or actor) role, much of the focus is geared towards workflow management
systems and their specification languages. The emphasis is on part of
business processing, namely process execution semantics: sequence, repetition,
choice, parallelism and synchronisation. A sound conceptualisation requires
not only this but also that process semantics, e.g.\ the messaging, database
updates and retrievals involved, to be explicitly captured.

In general, for the conceptual level, a plethora of techniques have emerged
under different paradigms, which integrated into well-formed methods, 
lead to integrated IS specifications.
Not surprisingly, a variety of approaches to workflow modelling and workflow 
implementation specifications exist
\cite{Article:94:Abbott:WFS}. 
Process modelling techniques allow basic features of business processes 
to be described through process classification, decomposition, control 
and data flow. The links to an organisational structure, e.g. actors and 
organisational units may be defined as process attributes
\cite{Article:91:Dur:TaskActor},
while specialisations of process classes define the processing structure, 
e.g.\ activities, tasks and actions as described in 
\cite{Book:88:Olle:Methodologies}. More advanced strategies are surveyed in
\cite{Article:92:Curtis:BusMod}.
In a similar fashion, object modelling techniques may also be adapted, 
e.g.\ in~\cite{Article:91:Antonellis:OOA},
a business process is modelled as an object type, and a lifecycle
of object states governed by state transition rules, defines business process
execution. More recently, communication-based techniques have been spawned 
by the work of
\cite{Article:80:Flores:ComMod}
based on the speech act theory of
\cite{Book:69:Searle:ComMod}.
These abstract workflows from organisational processing structure and 
use organisational communication - human interactions - as the focus. 
This provides a further insight into business process redesign and the
interactive aspects of workflows.

In absence of a universal organisational theory, the degree to which the
workflows are conceptualised for different organisational situations 
- indeed the degree to which techniques support a complete conceptualisation
- cannot be assessed theoretically. Rather, the adaption of techniques
for a synthesis of an organisational processing structure or organisation 
communication appears to adopt a \EM{constructivist} position
\cite{Report:96:Falkenberg:ConcFramework}.
That is, an objective world-view is, at best, discerned through subjective 
and evolvable modelling concepts. 
The use of business (or enterprise) models as a context for IS conceptual
models,
e.g.\ as recommended in
\cite{Article:91:Bubenko:BusMod,
Article:93:Jarke:ReqEng}
provides a basis for an \EM{inter-subjective} world-view. A business model 
describes an organisation's operational and strategic states, as defined 
by, and perceived throughout, the organisation. Concepts such as goals, 
objectives, business services, business processes (of various specialisations), 
events, actors and actor roles, and resources (information and material) 
have been used variously in the business models, e.g.\ those in integrated 
specification frameworks e.g.\ 
\cite{PhdThesis:93:Ramackers:BehaviourMod},
in CAiSE tools e.g.\ AD/CYCLE
\cite{Article:90:Mercurio:CAiSE},
and in requirements engineering methods, e.g.\
\cite{Article:95:Berztiss:ReqEng,%
Article:95:Loucopoulos:ReqEng,%
Article:94:Anton:ReqEng}.

The question then becomes, how adequate are conceptual modelling \EM{techniques}
at embodying inter-subjective world-views of business domains? This is
not a matter of socio-technical strategy, which as important as it is,
is an issue of method
\cite{Article:91:Avison:InfSystResearch}
rather than technique.
Nor is it a matter of merely qualifying fundamental modelling concepts (e.g.\ 
process) with organisational attributes (e.g.\ business service). 
Rather, the business processing semantics of a world-view need to be infused 
into the semantics of a technique such that a workflow may be expressed 
and communicated adequately using that technique. In this regard, a set of 
requirements which address the collective adequacy of conceptual modelling 
techniques, as derived from important principles of
\cite{Report:82:ISO:Concepts},
is considered useful.

First and foremost, in accordance with the \EM{Conceptualisation Principle},
a technique should abstract models away from infrastructural or implementation 
details, into the conceptual level, where details are described essentially. 
The focal aspects of business models and workflow specification languages can 
deflect and sometimes dictate the quality of conceptualisation. Conversely, 
following the \EM{One Hundred Percent Principle}, techniques should provide 
a sufficient \EM{expressive power} so that a full conceptualisation is in fact 
possible. A problem occurs when the expressiveness of a workflow specification 
language exceeds that of a technique to the point where only a partial 
conceptualisation results, and the remainder is addressed at the 
implementation level. This problem is known in software engineering jargon 
as the \EM{waterfall}. Such a disjointness of analysis precludes a sound 
understanding of the problem, leading to premature implementations. 
Conceptual models also need to be communicated and validated with 
a diverse set of stakeholders and so mechanisms are required for an 
effective \EM{comprehensibility}. An effective graphical presentation 
together with abstraction/decomposition mechanisms facilitates this.
At the same time, a \EM{formal foundation} is required to 
prevent interpretation ambiguities and to enable formal reasoning. That 
a recent survey on workflow technology
\cite{Article:95:Georgakopoulos:WFOverview}
cited the problem that ``workflow models and process methodologies do not
explicitly support the specification of what it means for a workflow to
be correct'' is symptomatic of a lack of formal semantics. Together with a
formal syntax, this constitutes formal foundation. Finally and most relatedly 
to world-views, since a ``silver bullet'' for all types of 
domains is considered unrealistic (see e.g.\
\cite{Article:87:Benyon:SystemAnalyst,%
Article:87:Brooks:SilverBullet,%
Article:83:Malouin:ISMethods}),
techniques should be \EM{suitable} for their problem domains. This means
a close connection between the modelling concepts and features, and those 
required by the domain.

The focus of this paper is on the \EM{business suitability} of techniques for
workflow modelling. Of course, to speak of a general business suitability is
vague since there are many types of organisations and many types of business 
processing
\cite{Book:85:Davis:MIS}.
Rather, particular attention is drawn to a specific type of (operational)
business processing which exhibits precise execution paths. As examples, 
the processing of insurance claims, bank loans and land conveyancing, are 
mission-critical in nature and are rarely undertaken without strict operational 
procedure. 
Also, multiple interactions with clients and external organisations are
typically needed to fulfill service requests.
Given their closer connection with database technology, workflow systems 
are considered more appropriate for this type of business processing over 
CSCW
\cite{Article:92:McCready:WFS,Article:95:Georgakopoulos:WFOverview}. 
These notions of business processing, workflow and workflow systems are 
assumed hereafter.
 
Following the constructivist approach, a number of \EM{integrated} 
conceptual modelling techniques - i.e.\ containing elements of data, 
process and behaviour perspectives 
\cite{Book:88:Olle:Methodologies}
- are assessed using the aforementioned requirements.
In this way, the business suitability of the techniques is understood from the 
overall context of their adequacy. 
A business processing world-view which nuances the intuitive 
semantics of business services and business processes 
is then used to focus a detailed business suitability diagnosis.
As a result, five business suitability principles are elicited. These relate to:
the organisational embedding of conceptual models; their validation 
through \EM{business transactions} as a scenario; the coordination of
business process execution through business services to avoid a violation of
the \EM{Information Hiding Principle}; the incorporation of sometimes neglected 
aspects, e.g.\ combining structural and behavioural aspects, temporal aspects
and human to computer interaction (HCI), to enhance a 
business transaction model's cognition; and the explicit treatment of 
operational error handling for a workflow's execution resilience.

The paper is organised as follows. In section~\ref{survey}, techniques 
characteristic of the different paradigms - structured
process modelling, object-oriented modelling, behavioural process modelling
and business-oriented modelling - are assessed. In section~\ref{new-principles},
the problems and business suitability principles are defined. In 
section~\ref{epilogue}, the paper is concludes with an epilogue.








